CASTing Your Model: Learning to Localize Improves Self-Supervised Representations

Recent advances in self-supervised learning (SSL) have largely closed the gap with supervised ImageNet pretraining. Despite their success these methods have been primarily applied to unlabeled ImageNet images, and show marginal gains when trained on larger sets of uncurated images. We hypothesize that current SSL methods perform best on iconic images, and struggle on complex scene images with many objects. Analyzing contrastive SSL methods shows that they have poor visual grounding and receive poor supervisory signal when trained on scene images. We propose Contrastive Attention-Supervised Tuning(CAST) to overcome these limitations. CAST uses unsupervised saliency maps to intelligently sample crops, and to provide grounding supervision via a Grad-CAM attention loss. Experiments on COCO show that CAST significantly improves the features learned by SSL methods on scene images, and further experiments show that CAST-trained models are more robust to changes in backgrounds.

==> figures/crop_ablations.tex <==
\begin{table}[t]
    \centering \footnotesize
    \setlength{\tabcolsep}{4pt}

    \begin{subfigure}[t]{\linewidth}
        \begin{tabularx}{\linewidth}{Xccll}
        \toprule
        Method & $\phi_1$ & $\phi_2$ & \vocclf{} & \inclf{}\\
        \midrule
        \mocococo{} (Default) & 0.0 & 0.0 & 66.9 & 46.5 \\
        \mocococo{} (Constrained) & 0.2 & 0.0 & 69.3\Rise{2.4} & \todo{46} \\
        \bottomrule
        \end{tabularx}
        \vspace{-3pt}
        \caption{Effect of transform on \mocococo{}}
        \label{subtab:crop1}
        \vspace{5pt}
    \end{subfigure}

    \begin{subfigure}[t]{\linewidth}
        \begin{tabularx}{\linewidth}{Xccll}
        \toprule
        Method & $\phi_1$ & $\phi_2$ & \vocclf{} & \inclf{}\\
        \midrule
        \mocococo{} + \qapp{} & 0.0 & 0.00 \\
        \mocococo{} + \qapp{} & 0.1 & 0.01 \\
        \mocococo{} + \qapp{} & 0.2 & 0.04 & 72.8 & 48.2\\
        \midrule
        \mocococo{} + \qapp{} & 0.1 & 0.00\\
        \mocococo{} + \qapp{} & 0.2 & 0.00 & 73.1 & 48.7 \\
        \bottomrule
        \end{tabularx}
        \vspace{-3pt}
        \caption{Effect of $\phi_1$ and $\phi_2$}
        \label{subtab:crop2}
        \vspace{5pt}
    \end{subfigure}

    \begin{subfigure}[t]{\linewidth}
        \begin{tabularx}{\linewidth}{Xcll}
        \toprule
        Method & Saliency Maps & \vocclf{} & \inclf{} \\
        \midrule
        \mocococo{} + \qapp{} & \usps{} & 73.1 & 48.7 \\
        \mocococo{} + \qapp{} & BASNet & 73.4 & 48.6\\
        \bottomrule
        \end{tabularx}
        \vspace{-3pt}
        \caption{Effect of better saliency maps}
        \label{subtab:crop3}
    \end{subfigure}

    \caption{
        \textbf{Ablations: Saliency-constrained Random Crop.}
    }
    \label{tab:crop_ablations}
\end{table}


==> sections/other_evaluation.tex <==
\section{Additional Evaluation (To be merged with previous section)}
\label{sec:other_eval}
% \vspace{-5pt}

\input{figures/backgrounds_describe.tex}
\input{figures/backgrounds_results.tex}

\subsection{Evaluation on Backgrounds Challenge Dataset}
The Backgrounds Challenge~\cite{xiao2020noise} aims to assess the background-robustness of image classification models by measuring their accuracy on images containing foreground objects superimposed on various background types (see \cite{xiao2020noise} for details on dataset construction). The dataset consists of 9 ImageNet classes with 450 test images per class. The evaluations are performed on eight foreground-background combinations summarized in Table~\ref{tab:backgrounds}. 

Since CAST forces a model to attend to specific object of interest during training, we expect a self-supervised model trained with CAST to be less dependent on background correlations for image classification as compared to a vanilla self-supervised model, and thus perform better on the Backgrounds Challenge.
\todo{Discuss results}
%. Original: Both foreground and background are unmodified (i.e. the image is unmodified), 2. Only-FG: The foreground is unmodified and the background is black, 3.    

\begin{figure*}[t]
    \begin{subfigure}[t]{\textwidth}
    \includegraphics[width=\textwidth]{figures/ssl_grounding_1.jpg}
    \caption{}
    \end{subfigure}
    \begin{subfigure}[t]{\textwidth}
    \includegraphics[width=\textwidth]{figures/ssl_grounding_2.jpg}
    \caption{}
    \end{subfigure}
    \begin{subfigure}[t]{\textwidth}
    \includegraphics[width=\textwidth]{figures/ssl_grounding_3.jpg}
    \caption{}
    \end{subfigure}
    \caption{Self-supervised Grounding.}
\end{figure*}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/IoU_plot.jpg}
    \caption{
        Plot showing that CAST improves the visual grounding}
    \label{fig:visual_grounding_plot}
\end{figure}

% \begin{figure}[h]
%     \includegraphics[width=\textwidth]{figures/IoU_plot.jpg}
%     \caption{Plot showing that CAST improves the visual grounding}
% \end{figure}


\begin{figure*}[t]
    \begin{subfigure}[t]{0.5\textwidth}
    \includegraphics[width=\textwidth]{figures/Downstream_grounding_1.jpg}
    \caption{}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\textwidth}
    \includegraphics[width=\textwidth]{figures/Downstream_grounding_3.jpg}
    \caption{}
    \end{subfigure}
    \begin{subfigure}[t]{0.5\textwidth}
    \includegraphics[width=\textwidth]{figures/Downstream_grounding_2.jpg}
    \caption{}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\textwidth}
    \includegraphics[width=\textwidth]{figures/Downstream_grounding_4.jpg}
    \caption{}
    \end{subfigure}
    \caption{Downstream task Grounding. Qualitative comparison of Grad-CAM attention maps from fully supervised networks and the self-supervised networks (MoCO and MoCO + CAST) on the Imagenet-1k classification task. We can see hat CASTed models tend to rely less on spurious correlations -- in (a) the CASTed model looks just at the player whereas both fully supervised model and MoCO rely on the regions corresponding to the baseball field and in (c), the CASTed model looks only at the lamp, while other models also rely on the table below. In (b), (d) we can see that CASTed models look at the whole extent of the category present in the image.}
\end{figure*}

% Grounding evaluation on pretraining task and Grounding evaluation on downstream models.

% (include qualitative evaluation on both)



==> utils/space_saver.tex <==
% A collection of dubious space saving macros
\parskip=5pt
\abovedisplayskip 3.0pt plus2pt minus2pt%
\belowdisplayskip \abovedisplayskip
\renewcommand{\baselinestretch}{1} % only use this one in emergencies

%Section spacing
\newcommand{\csection}[1]{
    \vspace{-0.11in}
    \section{#1}
    \vspace{-0.10in}
}

\newcommand{\csubsection}[1]{
    \vspace{-0.09in}
    \subsection{#1}
    \vspace{-0.08in}
}

\newcommand{\csubsubsection}[1]{
    \vspace{-0.06in}
    \subsubsection{#1}
    \vspace{-0.05in}
}


%caption/figure spacing
\setlength{\floatsep}{1ex plus 0ex minus 0.5ex}
\setlength{\textfloatsep}{3ex plus 0ex minus 0ex}
\setlength{\abovecaptionskip}{0ex plus 0ex minus 0ex}
\setlength{\belowcaptionskip}{0ex plus 0ex minus 0ex}
